VBFDD-Agent for Electric Vehicle Battery Fault Detection and Diagnosis: Descriptive Text Modeling of Battery Digital Signals

With the rapid proliferation of electric vehicles, the safety and reliability of lithium-ion batteries have become critical concerns. Effective anomaly detection is essential for ensuring safe battery operation. However, as battery systems and operating scenarios become increasingly complex, battery fault diagnosis and maintenance require stronger cross-domain adaptability and human-AI collaboration. Traditional fault detection and diagnosis methods are usually designed for specific scenarios and predefined workflows, making them less effective in complex real-world applications. To address the scarcity of open-source battery fault report corpora and the lack of unified maintenance knowledge representation, this study proposes a descriptive text modeling approach for battery signal reports. Monitoring signals, statistical features, anomaly records, and state assessment results are transformed into structured and readable natural language descriptions, forming a language corpus for battery health diagnosis and maintenance. Based on this corpus, we propose VBFDD-Agent, a vehicle battery fault detection and diagnosis agent for automotive-grade battery systems. VBFDD-Agent integrates descriptive battery-state texts, historical case retrieval, local maintenance manuals, and large language model reasoning to generate structured diagnostic results and maintenance recommendations. Experiments show that the proposed framework can accurately perform anomaly monitoring based on descriptive textual representations and provide flexible, efficient, and actionable maintenance suggestions. Expert evaluation further confirms the practical value of the generated recommendations. Overall, VBFDD-Agent extends traditional battery diagnosis from label prediction to interpretable and maintenance-oriented decision support.

==> Sections/Information/Authors.tex <==


\author[1]{Joey Chan}[style=chinese,orcid=0009-0004-8100-1546]\ead{sjtu_chan_joey@sjtu.edu.cn}
%第几作者
%%通讯作者星标

%\credit{Methodology, Writing - Original Draft, Validation, Visualization}

\author[1]{Zhen Chen}[style=chinese,orcid=0000-0003-2590-0307]\ead{chenzhendr@sjtu.edu.cn}\cormark[1]

\ead[url]{https://me.sjtu.edu.cn/teacher_directory1/chenzhen.html}
%\credit{Conceptualization, Investigation, Resources, Supervision}

\author[1]{Ershun Pan}[style=chinese,orcid=0000-0001-6026-9755]\ead{pes@sjtu.edu.cn}
\ead[url]{https://ieem.sjtu.edu.cn/szdy/2953.html}
%第几作者
\affiliation[1]{organization={Department of Industrial Engineering and Management, School of Mechanical Engineering, Shanghai Jiao Tong University, Shanghai 200240, China}}
\cortext[1]{Corresponding author}
%\credit{Project administration, Writing - Review & Editing}

==> Sections/Information/Bibs.tex <==

\addcontentsline{toc}{section}{Reference}
\renewcommand\refname{Reference}
\begin{thebibliography}{99}
\bibitem{ref41} Omrani, M. M., & Jannesari, H. (2019). Economic and environmental assessment of reusing electric vehicle lithium-ion batteries for load leveling in the residential, industrial and photovoltaic power plants sectors. Renewable and Sustainable Energy Reviews, 116, 109413.
\bibitem{ref42} Wang, H., Li, Y. F., & Zhang, Y. (2023). Bioinspired spiking spatiotemporal attention framework for lithium-ion batteries state-of-health estimation. Renewable and Sustainable Energy Reviews, 188, 113728.
\bibitem{ref40} Vykhodtsev, A. V., Jang, D., Wang, Q., Rosehart, W., & Zareipour, H. (2022). A review of modelling approaches to characterize lithium-ion battery energy storage systems in techno-economic analyses of power systems. Renewable and Sustainable Energy Reviews, 166, 112584.
\bibitem{ref38} Meng, H., & Li, Y. F. (2019). A review on prognostics and health management (PHM) methods of lithium-ion batteries. Renewable and Sustainable Energy Reviews, 116, 109405.
\bibitem{ref34} Finegan, D. P., Zhu, J., Feng, X., Keyser, M., Ulmefors, M., Li, W. & Cooper, S. J. (2021). The application of data-driven methods and physics-based learning for improving battery safety. Joule, 5(2), 316-329.
\bibitem{ref35} Dey, S., Perez, H. E., & Moura, S. J. (2017). Model-based battery thermal fault diagnostics: Algorithms, analysis, and experiments. IEEE Transactions on Control Systems Technology, 27(2), 576-587.
\bibitem{ref36} Marcicki, J., Onori, S., & Rizzoni, G. (2010, January). Nonlinear fault detection and isolation for a lithium-ion battery management system. In Dynamic Systems and Control Conference (Vol. 44175, pp. 607-614).
\bibitem{ref37} Wei, J., Dong, G., & Chen, Z. (2019). Lyapunov-based thermal fault diagnosis of cylindrical lithium-ion batteries. IEEE Transactions on Industrial Electronics, 67(6), 4670-4679.
\bibitem{ref22} Li, Da & Zhang, Lei & Zhang, Zhaosheng & Liu, Peng & Deng, Junjun & Wang, Qiushi & Wang, Zhenpo. (2023). Battery safety issue detection in real-world electric vehicles by integrated modeling and voltage abnormality. Energy. 284. 128438. 10.1016/j.energy.2023.128438.
\bibitem{ref16} Cherdo, Y., Miramond, B., Pegatoquet, A., & Vallauri, A. (2023). Unsupervised Anomaly Detection for Cars CAN Sensors Time Series Using Small Recurrent and Convolutional Neural Networks. Sensors, 23(11), 5013. MDPI AG. Retrieved from http://dx.doi.org/10.3390/s23115013
\bibitem{ref39} Zhang, X., Liu, P., Lin, N., Zhang, Z., & Wang, Z. (2023). A novel battery abnormality detection method using interpretable Autoencoder. Applied Energy, 330, 120312.
\bibitem{ref17} A. R. Javed, M. Usman, S. U. Rehman, M. U. Khan and M. S. Haghighi, "Anomaly Detection in Automated Vehicles Using Multistage Attention-Based Convolutional Neural Network," in IEEE Transactions on Intelligent Transportation Systems, vol. 22, no. 7, pp. 4291-4300, July 2021, doi: 10.1109/TITS.2020.3025875.
\bibitem{ref5} Zhou, Y., Liang, X., Zhang, W., Zhang, L., & Song, X. (2021). VAE-based deep SVDD for anomaly detection. Neurocomputing, 453, 131-140.
\bibitem{ref6} Z. Ghrib, R. Jaziri and R. Romdhane, "Hybrid approach for Anomaly Detection in Time Series Data," 2020 International Joint Conference on Neural Networks (IJCNN), Glasgow, UK, 2020, pp. 1-7, doi: 10.1109/IJCNN48605.2020.9207013.
\bibitem{ref7} Ruff, L., Vandermeulen, R., Goernitz, N., Deecke, L., Siddiqui, S. A., Binder, A., Müller, E. & Kloft, M. (2018, July). Deep one-class classification. In International conference on machine learning (pp. 4393-4402). PMLR.
\bibitem{ref4} Kingma, D., Salimans, T., Poole, B., & Ho, J. (2021). Variational diffusion models. Advances in neural information processing systems, 34, 21696-21707.
\bibitem{ref18} Zhang, Junfeng & Zhang, Hui & Zhang, Xiaoxiong. (2021). Power Consumption Predicting and Anomaly Detection Based on Transformer and K-Means. Frontiers in Energy Research. 9. 779587. 10.3389/fenrg.2021.779587.
\bibitem{ref19} Y. Wang, N. Masoud and A. Khojandi, "Real-Time Sensor Anomaly Detection and Recovery in Connected Automated Vehicle Sensors," in IEEE Transactions on Intelligent Transportation Systems, vol. 22, no. 3, pp. 1411-1421, March 2021, doi: 10.1109/TITS.2020.2970295.
\bibitem{ref2} Chen, Y., Tian, Y., Pang, G., & Carneiro, G. (2022, June). Deep one-class classification via interpolated gaussian descriptor. In Proceedings of the AAAI Conference on Artificial Intelligence (Vol. 36, No. 1, pp. 383-392).
\bibitem{ref8} Akcay, S., Atapour-Abarghouei, A., & Breckon, T. P. (2019). Ganomaly: Semi-supervised anomaly detection via adversarial training. In Computer Vision–ACCV 2018: 14th Asian Conference on Computer Vision, Perth, Australia, December 2–6, 2018, Revised Selected Papers, Part III 14 (pp. 622-637). Springer International Publishing.
\bibitem{ref33} Xia, X., Pan, X., Li, N., He, X., Ma, L., Zhang, X., & Ding, N. (2022). GAN-based anomaly detection: A review. Neurocomputing, 493, 497-535.
\bibitem{ref9} Kingma, D. P., & Welling, M. (2013). Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.
\bibitem{ref24} Radford, A., Metz, L., Chintala, S.: Unsupervised Representation Learning with Deep Convolutional Generative Adversarial Networks. In: ICLR (2016)
\bibitem{ref25} Gregor, Karol, Danihelka, Ivo, Graves, Alex, and Wierstra, Daan. Draw: A recurrent neural network for image generation. arXiv preprint arXiv:1502.04623, 2015.
\bibitem{ref23} H. Hojjati and N. Armanfard, "DASVDD: Deep Autoencoding Support Vector Data Descriptor for Anomaly Detection," in IEEE Transactions on Knowledge and Data Engineering, doi: 10.1109/TKDE.2023.3328882.
\bibitem{ref26} Goldstein, M., & Dengel, A.R. (2012). Histogram-based Outlier Score (HBOS): A fast Unsupervised Anomaly Detection Algorithm.
\bibitem{ref27} T. R. Bandaragoda, K. M. Ting, D. Albrecht, F. T. Liu and J. R. Wells, "Efficient Anomaly Detection by Isolation Using Nearest Neighbour Ensemble," 2014 IEEE International Conference on Data Mining Workshop, Shenzhen, China, 2014, pp. 698-705, doi: 10.1109/ICDMW.2014.70.
\bibitem{ref28} Weglarczyk, Stanislaw. (2018). Kernel density estimation and its application. ITM Web of Conferences. 23. 00037. 10.1051/itmconf/20182300037.
\bibitem{ref29} Hubert, M, Debruyne, M, Rousseeuw, PJ. Minimum covariance determinant and extensions. WIREs Comput Stat. 2018;10:e1421. https://doi.org/10.1002/wics.1421
\bibitem{ref30} Breunig, M. M., Kriegel, H. P., Ng, R. T., & Sander, J. (2000, May). LOF: identifying density-based local outliers. In Proceedings of the 2000 ACM SIGMOD international conference on Management of data (pp. 93-104).
\bibitem{ref31} Dreiseitl S, Osl M, Scheibböck C, Binder M. Outlier Detection with One-Class SVMs: An Application to Melanoma Prognosis. AMIA Annu Symp Proc. 2010 Nov 13;2010:172-6. PMID: 21346963; PMCID: PMC3041295.
\bibitem{ref32} Kingma, D. P., & Welling, M. (2013). Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.
\end{thebibliography}
